Elliptic Flow: A Study of Space-Momentum Correlations In Relativistic Nuclear Collisions

Here I review measurements of v2, the second component in a Fourier decomposition of the azimuthal dependence of particle production relative to the reaction plane in heavy-ion collisions. v2 is an observable central to the interpretation of the subsequent expansion of heavy-ion collisions. Its large value indicates significant space-momentum correlations, consistent with the rapid expansion of a strongly interacting Quark Gluon Plasma. Data is reviewed for collision energies from sqrt[sNN] = 2 to 200 GeV. Scaling observations and comparisons to hydrodynamic models are discussed.

==> models.tex <==
\section{Model Comparisons}

write this.
%\begin{figure}[hbt]
%\begin{center}
%\centerline{  \includegraphics[width=1.0\textwidth]{figures/knudsen_number_cgc.eps}}
%\caption{ Left panel: $v_2$ in Au+Au and Cu+Cu collisions scaled by
%  eccentricity calculated in a CGC framework and plotted
%  versus $(1/S)(dN/dy)$. The fit function and hydrodynamic limit are
%  explained in the text. Right panel: The effective Knudsen extracted
%  from the data and fit in the left panel.}
%  \label{fig:v2excitation}
%\end{center}
%\end{figure}

